Tracking Anything with Decoupled Video Segmentation

Training data for video segmentation are expensive to annotate. This impedes extensions of end-to-end algorithms to new video segmentation tasks, especially in large-vocabulary settings. To 'track anything' without training on video data for every individual task, we develop a decoupled video segmentation approach (DEVA), composed of task-specific image-level segmentation and class/task-agnostic bi-directional temporal propagation. Due to this design, we only need an image-level model for the target task (which is cheaper to train) and a universal temporal propagation model which is trained once and generalizes across tasks. To effectively combine these two modules, we use bi-directional propagation for (semi-)online fusion of segmentation hypotheses from different frames to generate a coherent segmentation. We show that this decoupled formulation compares favorably to end-to-end approaches in several data-scarce tasks including large-vocabulary video panoptic segmentation, open-world video segmentation, referring video segmentation, and unsupervised video object segmentation. Code is available at: https://hkchengrex.github.io/Tracking-Anything-with-DEVA

==> tabs/tab-app-vipseg-extended.tex <==
\centering
\begin{tabular}{l@{\hspace{1mm}}l@{\hspace{3mm}}l@{\hspace{3mm}}l@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}cc}
\toprule
Backbone & & & & VPQ$^1$ & VPQ$^2$ & VPQ$^4$ & VPQ$^6$ & VPQ$^{8}$ & VPQ$^{10}$ & VPQ$^\infty$ & $\overline{\text{VPQ}}$ & STQ\\
\midrule
Clip-PanoFCN & & end-to-end~\cite{miao2022large} & semi-online & 27.3/32.1/23.1 & 26.0/29.8/22.6 & 24.2/26.9/21.8 & 22.9/24.7/21.4 & 22.1/23.3/21.1 & 21.5/22.0/21.1 & 18.1/18.9/17.4 \\
Clip-PanoFCN & & decoupled (ours) & online & 29.5/35.3/24.3 & 28.9/34.5/24.0 & 28.1/33.3/23.5 & 27.2/32.1/23.0 & 26.7/31.2/22.7 & 26.1/30.2/22.4 & 25.0/28.9/21.7 \\
Clip-PanoFCN & & decoupled (ours) & semi-online & 31.3/36.7/26.5 & 30.8/35.9/26.3 & 30.1/34.8/25.9 & 29.4/33.7/25.6 & 28.8/32.8/25.3 & 28.3/31.9/25.1 & 27.1/30.4/24.2 \\
\midrule
Video-K-Net & R50 & end-to-end~\cite{li2022video} & online & 35.4 & 30.8 & 28.5 & 27.0 & 25.9 & 24.9 & 21.7 & 25.2 & 33.7 \\
Video-K-Net & R50 & decoupled (ours) & online & 35.8 & 35.2 & 34.5 & 33.6 & 33.1 & 32.6 & 30.5 & 32.3 & 38.4 \\
Video-K-Net & R50 & decoupled (ours) & semi-online & 37.1 & 36.5 & 35.8 & 35.1 & 34.7 & 34.3 & 32.3 & 33.9 & 38.6 \\
Mask2Former & R50 & decoupled (ours) & online & 41.0 & 40.2 & 39.3 & 38.4 & 37.9 & 37.3 & 33.8 & 36.4 & 41.1 \\
Mask2Former & R50 & decoupled (ours) & semi-online & \textbf{42.1} & \textbf{41.5} & \textbf{40.8} & \textbf{40.1} & \textbf{39.7} & \textbf{39.3} & \textbf{36.1} & \textbf{38.3} & \textbf{41.5} \\
\midrule
Video-K-Net & Swin-B & end-to-end~\cite{li2022video} & online & 49.8 & 45.2 & 42.4 & 40.5 & 39.1 & 37.9 & 32.6 & 37.5 & 45.2 \\
Video-K-Net & Swin-B & decoupled (ours) & online & 48.2 & 47.4 & 46.5 & 45.6 & 45.1 & 44.5 & 42.0 & 44.1 & 48.6 \\
Video-K-Net & Swin-B & decoupled (ours) & semi-online & 50.0 & 49.3 & 48.5 & 47.7 & 47.3 & 46.8 & 44.5 & 46.4 & 48.9 \\
Mask2Former & Swin-B & decoupled (ours) & online & 55.3 & 54.6 & 53.8 & 52.8 & 52.3 & 51.9 & 49.0 & 51.2 & \textbf{52.4} \\
Mask2Former & Swin-B & decoupled (ours) & semi-online & \textbf{56.0} & \textbf{55.4} & \textbf{54.6} & \textbf{53.9} & \textbf{53.5} & \textbf{53.1} & \textbf{50.0} & \textbf{52.2} & 52.2 \\
\midrule
\bottomrule
\end{tabular}


==> tabs/tab-app-vos-2.tex <==
\centering
\begin{tabular}
{l@{\hspace{10pt}}C{2.2em}@{}C{2.2em}@{}C{2.2em}}
\toprule
& \multicolumn{3}{c}{DAVIS-17 test-dev} \\
\cmidrule(lr{\dimexpr 4\tabcolsep+12pt}){2-5} 
Method & \mjf & \mj & \mf \\
\midrule
STCN~\cite{xu2021rethinking} & 52.5 & 48.5 & 56.6 \\
AOT-R50~\cite{yang2021associating} & 58.4 & 54.3 & 62.6 \\
XMem~\cite{cheng2022xmem} & 56.3 & 52.1 & 60.6 \\
DEVA (ours), w/o OVIS & 60.0 & 55.8 & 64.3 \\
DEVA (ours), w/ OVIS & 66.5 & 62.3 & 70.8 \\
\midrule
\bottomrule
\end{tabular}

==> tabs/tab-association.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}c}
    \toprule
    Variant & VPQ$^1$ & VPQ$^2$ & VPQ$^4$ & VPQ$^6$ & VPQ$^{8}$ & VPQ$^{10}$ & VPQ$^\infty$ & $\overline{\text{VPQ}}$ & STQ\\
    \midrule
    Ours, full model & \textbf{40.9} & \textbf{40.3} & \textbf{39.6} & \textbf{39.1} & \textbf{38.6} & \textbf{38.2} & \textbf{35.2} & \textbf{37.3} & \textbf{42.4} \\
    \toprule
    \midrule
    Hungarian matching on IoU & 39.8 & 35.6 & 32.0 & 29.2 & 27.1 & 25.3 & 17.9 & 24.7 & 34.5 \\
    Hungarian matching on IoU + flow~\cite{teed2020raft} &  40.2 & 36.6 & 33.1 & 30.4 & 28.3 & 26.5 & 19.3 & 25.9 & 37.0 \\
    Hungarian matching on object queries (MinVIS~\cite{huang2022minvis}) & 40.4 & 36.0 & 32.2 & 29.3 & 27.1 & 25.2 & 17.9 & 24.8 & 35.8 \\
    \toprule
    \midrule
    Replace instead of merge & 39.5 & 38.3 & 37.0 & 36.0 & 35.3 & 34.7 & 31.1 & 34.0 & 40.2 \\
    Replace instead of merge, re-init internal memory & 39.8 & 37.9 & 35.8 & 33.8 & 32.6 & 31.5 & 26.8 & 31.0 & 37.5 \\
    \midrule
    No refinement & 40.2 & 39.5 & 38.6 & 37.9 & 37.4 & 36.8 & 33.1 & 35.8 & 42.0 \\
    \midrule
    \bottomrule
    \end{tabular}
    \vspace{-0.8em}
    \caption{Ablations on the VIPSeg~\cite{miao2022large} dataset. All variants use Mask2Former-R50 as the image model. Top: our generalized mask propagation approach performs better than pure association-based methods. Bottom: both merging and refinement are beneficial to our final high performance. In both cases, the effects are especially prominent in the long-term with large $k$.}
    \label{tab:association}
    \vspace{-1.2em}
\end{table*}
